Douglas-Rachford splitting and ADMM for nonconvex optimization: tight convergence results

Although originally designed and analyzed for convex problems, the alternating direction method of multipliers (ADMM) and its close relatives, Douglas-Rachford splitting (DRS) and Peaceman-Rachford splitting (PRS), have been observed to perform remarkably well when applied to certain classes of structured nonconvex optimization problems. However, partial global convergence results in the nonconvex setting have only recently emerged. In this paper we show how the Douglas-Rachford envelope (DRE), introduced in 2014, can be employed to unify and considerably simplify the theory for devising global convergence guarantees for ADMM, DRS and PRS applied to nonconvex problems under less restrictive conditions, larger prox-stepsizes and over-relaxation parameters than previously known. In fact, our bounds are tight whenever the over-relaxation parameter ranges in $(0,2]$. The analysis of ADMM uses a universal primal equivalence with DRS that generalizes the known duality of the algorithms.

==> TeX/Text/ADMM/Image.tex <==
The notion of \emph{image function}, also known as \emph{epi-composition} or \emph{infimal post-composition} \cite{auslender2002asymptotic,bauschke2017convex,rockafellar2011variational} will play an important role in \Cref{sec:ADMM}.
\begin{defin}[Image function]\label{defin:epicomp}%
	Given \(\func{h}{\R^n}{\Rinf}\) and \(C\in\R^{m\times n}\), the \DEF{image function} \(\func{\epicomp Ch}{\R^m}{[-\infty,+\infty]}\)
% 	(also known as \DEF{epi-composition} or \DEF{infimal postcomposition})
	is defined as
	\[
		\epicomp Ch(s)
	{}\coloneqq{}
		\inf_{x\in\R^n}\set{h(x)}[Cw=s].
	\]
\end{defin}

% \begin{lem}
% 	For any \(\func{h}{\R^n}{\Rinf}\), \(C\in\R^{p\times n}\), and \(\gamma>0\) it holds that
% 	\[
% 		\prox_{\gamma\epicomp Ch}
% 	{}={}
% 		C\argmin_{x\in\R^n}\set{h(x)+\tfrac{1}{2\gamma}\|Ax-{}\cdot{}\|^2}.
% 	\]
% 	\begin{proof}
% 		\begin{align*}
% 				\bar s
% 			{}\in{}
% 				\prox_{\gamma\epicomp Ch}(s)
% 		{}\Leftrightarrow{} &
% 				\epicomp Ch(\bar s)
% 				{}+{}
% 				\tfrac{1}{2\gamma}\|\bar s-s\|^2
% 			{}\leq{}
% 				\epicomp Ch(s')
% 				{}+{}
% 				\tfrac{1}{2\gamma}\|\bar s-s'\|^2
% 		&
% 			\forall s'\in\R^p
% 		\\
% 		{}\Leftrightarrow{} &
% 				\epicomp Ch(\bar s)
% 				{}+{}
% 				\tfrac{1}{2\gamma}\|\bar s-s\|^2
% 			{}\leq{}
% 				\epicomp Ch(Cx')
% 				{}+{}
% 				\tfrac{1}{2\gamma}\|\bar s-Cx'\|^2
% 		&
% 			\forall x'\in\R^n
% 		\end{align*}
% % 		{}={}
% % 			C\argmin_{x\in\R^n}\set{h(x)+\tfrac{1}{2\gamma}\|Ax-{}\cdot{}\|^2}.
% % 		{}={}
% % 			C\argmin_{x\in\R^n}\set{h(x)+\tfrac{1}{2\gamma}\|Ax-{}\cdot{}\|^2}.
% % 		\end{align*}
% 
% 		Fix \(\bar s\in\R^p\), and let \(x_\beta\in X_\beta(\bar s)\).
% 		Then, from \ref{thm:epiexact} and the optimality of \(x_\beta\) we have
% 		\[
% 			\epicomp Ch(Cx_\beta)
% 			{}+{}
% 			\tfrac\beta2\|Cx_\beta-\bar s\|^2
% 		{}={}
% 			h(x_\beta)
% 			{}+{}
% 			\tfrac\beta2\|Cx_\beta-\bar s\|^2
% 		{}\leq{}
% 			h(x)
% 			{}+{}
% 			\tfrac\beta2\|Cx-\bar s\|^2
% 		\]
% 		for all \(x\in\R^n\).
% 		In particular, this holds for all \(s\in\R^p\) and \(x\) such that \(Cx=s\), hence
% 		\[
% 			\epicomp Ch(Cx_\beta)
% 			{}+{}
% 			\tfrac\beta2\|Cx_\beta-\bar s\|^2
% 		{}\leq{}\!
% 			\inf_{x:Cx=s}\set{
% 				h(x)
% 				{}+{}
% 				\tfrac\beta2\|Cx-\bar s\|^2
% 			}
% 		{}={}
% 			\epicomp Ch(s)
% 			{}+{}
% 			\tfrac\beta2\|s-\bar s\|^2
% 		\]
% 		proving
% 		\(
% 			CX_\beta(\bar s)
% 		{}\subseteq{}
% 			\prox_{\nicefrac{\epicomp Ch}{\beta}}(\bar s)
% 		\).
% 		Similar reasonings yield the other inclusion too.
% 	\end{proof}
% \end{lem}
\begin{prop}\label{thm:lsc}%[Condition for lsc of image function]\label{thm:lsc}%
	Let \(\func{h}{\R^n}{\Rinf}\) and \(C\in\R^{p\times n}\).
	Suppose that for some \(\beta>0\) the set-valued function \(\ffunc{X_\beta}{\R^p}{\R^n}\) defined by
% 	\begin{equation}\label{eq:Xb(s)}
	\(
		X_\beta(s)
	{}\coloneqq{}
		\argmin_{x\in\R^n}\set{
			h(x)+\tfrac\beta2\|Cx-s\|^2
		}
	\),
% 	\end{equation}
	is nonempty for all \(s\in\R^p\).
	Then,
	\begin{enumerate}
	\item\label{thm:epiproper}%
		The image function \(\epicomp Ch\) is proper.
	\item\label{thm:epiexact}%
		\(
			\epicomp Ch(Cx_\beta)
		{}={}
			h(x_\beta)
		\)
		for all \(s\in\R^p\) and
		\(
			x_\beta
		{}\in{}
			X_\beta(s)
		\).
	\item\label{thm:AX}%
		\(
			\prox_{\nicefrac{\epicomp Ch}{\beta}}\supseteq CX_\beta
		\).
	\note{Can't we have the other inclusion?}%
\grayout{%
			and in particular the set-valued map \(s\mapsto CX_\beta(s)\) is locally bounded;
			\item\label{thm:penalty}%
				\(
					\tfrac\beta2\|Cx_\beta-\bar s\|^2\to 0
				\)
				as \(\beta\to\infty\), for any \(x_\beta\in X_\beta(\bar s)\);
			\item\label{thm:epilsc}%
				\(\epicomp Ch\) is lsc at \(\bar s\) iff
				\(
					h(x_\beta)\to\epicomp Ch(\bar s)
				\)
				as
				\(
					\beta\to\infty
				\),
				where \(x_\beta\in X_\beta(\bar s)\).
}%
	\end{enumerate}
	\begin{proof}
		See \Cref{proof:thm:lsc}.
	\end{proof}
\end{prop}
\begin{prop}\label{thm:epipartial}%
	For a function \(\func{h}{\R^n}{\Rinf}\) and \(C\in\R^{p\times n}\), let \(\ffunc X{\R^p}{\R^n}\) be defined as
% 	\begin{equation}\label{eq:X(s)}
	\(
		X(s)
	{}\coloneqq{}
		\argmin_{x\in\R^n}\set{h(x)}[Cx=s]
	\).
% 	\end{equation}
	Then, for all \(\bar s\in C\dom h\) and \(\bar x\in X(\bar s)\) it holds that
	\[
		\trans C\hat\partial\epicomp Ch(\bar s)
% 	{}={}
% 		\trans C\hat\partial\epicomp Ch(C\bar x)
	{}\subseteq{}
		\hat\partial h(\bar x).
	\]
% 	In particular, if \(C\) is surjective (full-row rank) and \(h\) is differentiable at \(\bar x\), then \(\hat\partial\epicomp Ch(C\bar x)\) is either empty or a singleton.
	\begin{proof}
		See \Cref{proof:thm:epipartial}.
	\end{proof}
\end{prop}

\begin{prop}[Strong convexity of the image function]\label{thm:epicompStrCvx}%
	Suppose that \(\func h{\R^n}{\Rinf}\) is proper, lsc, and \(\sigma_h\)-strongly convex.
	Then, for every \(C\in\R^{p\times n}\) the image function \(\epicomp Ch\) is \(\sigma_{\epicomp Ch}\)-strongly convex with \(\sigma_{\epicomp Ch}=\nicefrac{\sigma_h}{\|C\|^2}\)
	\begin{proof}
		See \Cref{proof:thm:epicompStrCvx}
	\end{proof}
\end{prop}


\grayout{%
	In order to proceed to the next result, we first need to introduce the following important notion for parametric minimization.
	\begin{defin}[Locally uniform level boundedness {\cite[Def. 1.16]{rockafellar2011variational}}]\label{defin:ULB}%
		We say that a function \(\func{M}{\R^m\times\R^n}{\Rinf}\) with values \(M(w,x)\) is \DEF{level bounded in \(w\) locally uniformly in \(x\)} if for all \(\alpha\in\R\) and \(\bar x\in\R^n\) there exists \(\varepsilon>0\) such that the set
		\[
			\set{(w,x)\in\R^m\times\R^n}[
				M(w,x)\leq\alpha,~
				\|x-\bar x\|\leq\varepsilon
			]
		\]
		is bounded.
	\end{defin}

	\begin{thm}\label{thm:epicompLB}%
		Let \(\func{h}{\R^n}{\Rinf}\) be lsc and \(C\in\R^{p\times n}\).
		Suppose that for some \(\beta>0\) the function \(h+\tfrac\beta2\|C{}\cdot{}-s\|^2\) is level bounded for all \(s\in\R^p\).
		Then, the following hold:
		\begin{enumerate}
		\item
			\(\epicomp Ch\) is proper and lsc.
		\item
			For all \(s\in C\dom h\) the set of minimizers \(X(s)\) as in \eqref{eq:X(s)} is nonempty; moreover, \(X\) is locally bounded, and it is osc with respect to \(\epicomp Ch\)-attentive convergence: for all \(\bar s\in C\dom h\)
			\[
				\limsup_{k\to\infty}X(s_k)
			{}\subseteq{}
				X(\bar s)
			\]
			whenever \(\bigl(s^k,\epicomp Ch(s^k)\bigr)\to\bigl(\bar s,\epicomp Ch(\bar s)\bigr)\) as \(k\to\infty\).
		\item
			For all \(\bar s\in C\dom h\) and \(\bar x\in X(\bar s)\) one has
			\[
				\trans C\partial\epicomp Ch(\bar s)
			{}\subseteq{}
				\bigcup_{\bar x\in X(\bar s)}{
					\partial h(\bar x)
				}.
			\]
		\end{enumerate}
		\begin{proof}
			The level boundedness condition ensures that 
			\(
				H(x,s)
			{}\coloneqq{}
				h(x)+\indicator_{\set0}(Cx-s)
			\)
			is level bounded in \(x\), locally uniformly in \(s\), cf. \cref{defin:ULB}.
			The first two claims then follow from \cite[Thm. 1.32]{rockafellar2011variational}.
			
			Let \(\bar v\in\partial\epicomp Ch(\bar s)\) be fixed.
			Then, there exits a sequence \(\seq{s^k,v^k}\subseteq\graph\hat\partial h\) such that
			\(
				\bigl(
					s^k,
					\epicomp Ch(s^k),
					v^k
				\bigr)
			{}\to{}
				\bigl(
					\bar s,
					\epicomp Ch(\bar s),
					\bar v
				\bigr)
			\)
			as \(k\to\infty\).
			For each \(k\in\N\) let \(x^k\in X(s^k)\); then, \(\seq{x^k}\) is bounded and all its accumulation points belong to \(X(\bar s)\); thus, up to possibly extracting, \(x^k\to\bar x\) for some \(\bar x\in X(\bar s)\) as \(k\to\infty\).
			Then,
			\[
				\trans C\bar v
			{}={}
				\lim_{k\to\infty}{
					\trans Cv^k
				}
			{}\overrel*[\in]{\ref{thm:epipartial}}[2pt]{}
				\limsup_{k\to\infty}{
					\hat\partial h(x^k)
				}
			{}\subseteq{}
				\partial h(\bar x),
			\]
			where the last inclusion follows from the definition of \(\partial h\) and the fact that
			\[
				h(x^k)
			{}={}
				\epicomp Ch(s^k)
			{}\to{}
				\epicomp Ch(\bar s)
			{}={}
				h(\bar x).
			\]
			The claimed inclusion then follows from the arbitrarity of \(\bar v\in\partial\epicomp Ch(\bar s)\).
		\end{proof}
	\end{thm}


	\begin{lem}\label{thm:epicomp:convex}%
		Let \(\func h{\R^n}{\Rinf}\) be convex and \(C\in\R^{p\times n}\) be surjective.
		Then, \(\epicomp Ch\) is convex, and as long as the set of minimizers \(X(\bar s)\) is nonempty (see \eqref{eq:X(s)}), it holds that
		\[
			\partial\epicomp Ch(\bar s)
		{}={}
			\set{y}[\trans Ay\in\partial h(\bar x)],
		\]
		where \(\bar x\) is any element of \(X(\bar s)\).
		In particular, if \(h\) is differentiable at some point in \(X(\bar s)\), then \(\epicomp Ch\) is differentiable at \(\bar s\).
		\begin{proof}
			See \cite[Thm. D.4.5.1 and Cor. D.4.5.2]{hiriarturruty2012fundamentals}.
		\end{proof}
	\end{lem}
}%


==> TeX/Text/DRE/Regularity.tex <==
% The interested reader is referred to \cite{rockafellar2011variational} for an extensive discussion on these notions.
\begin{thm}[Local continuous differentiability]\label{prop:C1}%
	Let \(\bar s\) be a fixed point for the \ref{DRS} iterations with stepsize \(\bar\gamma\) and let \(\bar u=\prox_{\gamma\sDRS}(\bar s)\).
	Suppose that the following hold:
	\begin{enumerate}
	\item
		\(\restr{\sDRS}\) is \(\cont^2\) around \(\bar s\), and
	\item
		\(\nsDRS\) is prox-regular at \(\bar u\) for \(-\Nabla\sDRS(\bar u)\) in the sense of \cite[Def. 13.27]{rockafellar2011variational}.
	\end{enumerate}
	Then, for all \(\gamma\in(0,\bar\gamma)\) there exists a neighborhood \(\mathcal U\) of \(\bar u+\gamma\Nabla\sDRS(\bar u)\) such that \(\DRE\in\cont^1(\mathcal U)\), with
	\[
		\nabla\DRE(s)
	{}={}
		\tfrac1\gamma
		J\prox_{\gamma\sDRS}(s)
		Q_\gamma(u)
		(u-v)
	\qquad\text{for all }
		s\in\mathcal U,
	\]
	where
	\(
		Q_\gamma
	{}\coloneqq{}
		\I-\gamma\Nabla^2\sDRS
	\)
	and \(u\) and \(v\) are as in \eqref{DRS}.
	\begin{proof}
		Since
		\(
			0
		{}\in{}
			\Res[\gamma][FB](\bar u)
		\)
		(cf. \eqref{eq:Res}), it follows from \cite[Thm. 4.7]{themelis2016forward} that for all \(\gamma<\bar\gamma\) the FBE \(\FBE\) is of class \(\cont^1\) in a neighborhood of \(\bar u\) with
		\[
			\nabla\FBE(u)
		{}={}
			\tfrac1\gamma
			Q_\gamma(u)
			\Res[\gamma][FB](u)
		{}={}
			\tfrac1\gamma
			Q_\gamma(u)
			(u-v).
		\]
		Moreover, we know from \cref{prop:proxfC1} that \(\prox_{\gamma\sDRS}\) is \(\cont^1\) around \(\bar u+\gamma\Nabla\sDRS(\bar u)\).
		The proof now follows from the chain rule of differentiation applied to
		\(
			\DRE
		{}={}
			\FBE\circ\prox_{\gamma\sDRS}
		\).
	\end{proof}
\end{thm}

In the convex setting, being a fixed point is a property independent of the stepsize \(\gamma\), and as such the value of the stepsize \(\gamma\) plays no role in \Cref{prop:C1}.
On the contrary, for nonconvex problems ruling out \(\gamma=\bar\gamma\) is a necessary condition for ensuring differentiability of the DRE.
To see this, consider \(\varphi=\func{\sDRS+\nsDRS}{\R}{\Rinf}\) for \(\sDRS(x)=\tfrac12x^2\) and \(\nsDRS=\indicator_{\set{0,1}}\).
A simple verification shows that \(\nsDRS\) is prox-regular on its domain for all subgradients and that \(\bar s=\nicefrac32\) is a fixed point for \ref{DRS} with stepsize \(\gamma=\nicefrac12\).
Observe that
\(
	\bar u
{}\coloneqq{}
	\prox_{\nicefrac{\sDRS}{2}}(\bar s)
{}={}
	1
\)
and that the DRE
\[
	\DRE(s)
{}={}
	\tfrac{1-\gamma}{2(1+\gamma)^2}s^2
	{}+{}
	\tfrac{1}{2\gamma}
	\dist\bigl(
		\tfrac{1-\gamma}{1+\gamma}s,\,\set{0,1}
	\bigr)^2
\]
is differentiable at
\(
	s_\gamma
{}\coloneqq{}
	\bar u
	{}+{}
	\gamma\Nabla\sDRS(\bar u)
{}={}
	1+\gamma
\)
for all \(\gamma<\nicefrac12\) but fails to be so for \(\gamma=\nicefrac12\).
This pathology is due to the fact that while \(\Res(s_\gamma)=\set 0\) for all \(\gamma<\nicefrac12\), for \(\gamma=\nicefrac12\) the residual is not single valued.
The following result clarifies these claims; the interested reader is referred to the more detailed analysis in \cite[§3]{themelis2016forward} which deals with similar issues of forward-backward iterations.
\begin{prop}[Regularity of fixed points]\label{prop:fix}%
	Suppose that \(\bar s\in\dom\sDRS\) is a fixed point for the \ref{DRS} iterations with stepsize \(\bar\gamma\) and let \(\bar u=\prox_{\bar\gamma\nsDRS}(\bar s)\).
	Then, for all \(\gamma<\bar\gamma\) the point \(s_\gamma=\bar u+\gamma\Nabla\sDRS(\bar u)\) (\ie such that \(\prox_{\gamma\sDRS}(s)=\bar u\)) is a fixed point and, additionally, \(\Res(s)=\set0\) (instead of merely \(0\in\Res(s)\)).
	\begin{proof}
		That \(\prox_{\gamma\sDRS}(s)=\bar u\) follows from	\cref{prop:proxfEquiv} and the fact that \(s\in\dom\sDRS\).
		Due to \eqref{eq:vFBS}, the claim reduces to showing that \(\FB{\bar u}=\set u\) for all \(\gamma<\bar\gamma\), which is proven in \cite[Thm. 3.4{\it(iii)}]{themelis2016forward}.
	\end{proof}
\end{prop}



==> TeX/Text/DRE/SD.tex <==
We now study the last fundamental property of the DRE, namely that for suitable values of \(\gamma\) and \(\lambda\) a sufficient decrease on \(\DRE\) can be enforced with a full \ref{DRS} update \(s\mapsto s^+\).
This will be the key result for ensuring convergence of \ref{DRS} for small enough stepsizes.
For this reason we are only interested in the case \(\gamma<\nicefrac{1}{L_{\sDRS}}\), for otherwise the DRE is not tightly related to the original cost, as \Cref{es:DREunbounded} demonstrates.
However, the bound \(\gamma<\nicefrac{1}{L_{\sDRS}}\) is necessary for ensuring the convergence of \ref{DRS}, unless the generality of \Cref{ass:fg} is sacrificed.
This claim will be shown in \Cref{sec:DRS} by means of suitable counterexamples.
\begin{thm}[Sufficient decrease]\label{thm:SD}%
	Consider one \ref{DRS} update
	\(
		s
	{}\mapsto{}
		(u,v,s^+)
	\)
	for some relaxation \(\lambda\in(0,2)\) and feasible stepsize
	\(
		\gamma
	{}<{}
		\min\set{
			\tfrac{2-\lambda}{2[\sigma_{\sDRS}]_-},\,
			\tfrac{1}{L_{\sDRS}}
		}
	\).
	Then,
	\begin{equation}\label{eq:SD}
		\DRE(s)-\DRE(s^+)
	{}\geq{}
		c\,
		\|u-v\|^2
	\end{equation}
	where \(c\) is a strictly positive constant defined as
	\[
		c
	{}\coloneqq{}
		\tfrac{\lambda}{(1+\gamma L_{\sDRS})^2}
		\left(
			\tfrac{2-\lambda}{2\gamma}
			{}-{}
			\max\set{
				[\sigma_{\sDRS}]_-,\,\,
				L_{\sDRS}(\gamma L_{\sDRS}\!-\tfrac\lambda2)
				\vphantom{\Big|}
			}
		\right).
	\]
	If \(\sDRS\) is strongly convex then \eqref{eq:SD} also holds for
	\(
		2
	{}\leq{}
		\lambda
	{}<{}
		\tfrac{4}{1+\sqrt{1-p_{\sDRS}}}
	\)~
	and feasible \(\gamma\) such that~
	\(
		\tfrac{
			p_{\sDRS}\lambda
			{}-{}
			\delta
		}{
			4\sigma_{\sDRS}
		}
	{}<{}
		\gamma
	{}<{}
		\tfrac{
			p_{\sDRS}\lambda
			{}+{}
			\delta
		}{
			4\sigma_{\sDRS}
		}
	\),~
	where\ 
	\(
		\delta
	{}\coloneqq{}
		\sqrt{(p_{\sDRS}\lambda)^2-8p_{\sDRS}(\lambda-2)}
	\),~
	in which case
	\[
		c
	{}\coloneqq{}
		\tfrac{\lambda}{(1+\gamma L_{\sDRS})^2}
		\left(
			\tfrac{2-\lambda}{2\gamma}
			{}+{}
			\sigma_{\sDRS}
			(\tfrac\lambda2-\gamma L_{\sDRS})
		\right).
	\]
\end{thm}
For the sake of readability, the proof of \Cref{thm:SD} is referred to the dedicated \Cref{sec:proof:SD}.
In the most common cases \(\lambda=1\) and \(\lambda=2\), \ie classical (non relaxed) DRS and PRS respectively, the bounds on \(\gamma\) can be simplified as follows.
\begin{rem}[Special cases: DRS \& PRS]\label{rem:DRS}%
	Merely distinguishing between convex and nonconvex smooth function \(\sDRS\), \ie with either \(\sigma_{\sDRS}=-L_{\sDRS}\) or \(\sigma_{\sDRS}=0\), the range of \(\gamma\) and the sufficient decrease constant \(c\) can be simplified as follows:
	\begin{itemize}
	\item
		\(\lambda=1\): Douglas-Rachford splitting
		\[
			\begin{cases}[%
				@{\gamma<{}} l
				@{~~\text{and}~~c={}\tfrac{1}{(1+\gamma L_{\sDRS})^2}} l
				@\quad l%
			]
				\frac{1}{L_{\sDRS}}
			&
				\tfrac{
					1
					{}-{}
					\gamma L_{\sDRS}
					[2\gamma L_{\sDRS}-1]_+
				}{2\gamma}
			&
				\text{if \(\sDRS\) is convex,}
			\\[5pt]
				\frac{1}{2L_{\sDRS}}
			&
				\tfrac{
					1-2\gamma L_{\sDRS}
				}{2\gamma}
			&
				\text{otherwise.}
			\end{cases}
		\]
	\end{itemize}
	When it comes to PRS, the smooth function \(\sDRS\) must be strongly convex (\ie \(\sigma_{\sDRS}>0\)), in which case we have
	\begin{itemize}
	\item
		\(\lambda=2\): Peaceman-Rachford splitting (only for strongly convex \(\sDRS\))
		\begin{qedequation}
			\gamma
		{}<{}
			\tfrac{1}{L_{\sDRS}}
			~\text{ (regardless of \(\sigma_{\sDRS}\)) ~and }~
			c
		{}={}
			2\sigma_{\sDRS}
			\tfrac{1-\gamma L_{\sDRS}}{(1+\gamma L_{\sDRS})^2}.
		\end{qedequation}
	\end{itemize}\let\qed\relax%
\end{rem}












\begin{thm}[Subsequential convergence]\label{thm:DRS}%
	Suppose that the cost function \(\varphi\) is lower bounded.
	Then, the following hold for the iterates generated by \ref{DRS} with stepsize \(\gamma\) and relaxation \(\lambda\) as in \Cref{thm:SD}:
	\begin{enumerate}
	\item\label{thm:DRS:r}
		the sequence of DR-residuals \(\seq{u^k-v^k}\) is square-summable;
	\item\label{thm:DRS:uv}
		\(\seq{u^k}\) and \(\seq{v^k}\) have same cluster points, all of which are stationary for \(\varphi\) and on which \(\varphi\) has same value, this being the limit of \(\seq{\DRE(s^k)}\).
	\end{enumerate}
	Moreover, a sufficient condition for the sequences to be bounded is that \(\varphi\) has bounded level sets.
	\begin{proof}
		To avoid trivialities, we assume that the stopping criterion \(v^k=u^k\) is never met, so that the algorithm runs infinite many iterations.
		\begin{proofitemize}
		\item\ref{thm:DRS:r}
			Let \(c=c(\gamma,\lambda)\) be as in \cref{thm:SD}.
			Telescoping the inequality \eqref{eq:SD} yields
			\begin{align*}
			\textstyle
				c
				\sum_{k\in\N}{
					\|u^k-v^k\|^2
				}
			{}\leq{} &
			\textstyle
				\sum_{k\in\N}{
				\bigl[
					\DRE(s^k)
					{}-{}
					\DRE(s^{k+1})
				\bigr]}
			{}\leq{}
				\DRE(s^0)-\inf\DRE.
			\end{align*}
			Since \(\inf\DRE=\inf\varphi\) and \(\DRE\) is real-valued (cf. \cref{prop:C0,prop:DREequiv}), from the inequality above it follows that if \(\varphi\) is lower bounded then \(\seq{u^k-v^k}\) is square-summable.
			Moreover, since \(\DRE(s^k)\) is decreasing it admits a limit, be it \(\varphi_\star>-\infty\).
	%%%%%%%%
		\item\ref{thm:DRS:uv}
			Since \(\seq{u^k-v^k}\to 0\), necessarily \(\seq{u^k}\) and \(\seq{v^k}\) have same cluster points.
			From \cref{prop:proxfEquiv} it follows that for all \(k\in\N\)
			there exists \(\nu^k\in\dom\sDRS^\perp\) such that
			\(
				s^k
			{}={}
				u^k+\gamma\Nabla\sDRS(u^k)+\nu^k
			\).
% 			However, since
% 			\(
% 				v^k
% 			{}\in{}
% 				\dom\nsDRS
% 			{}\subseteq{}
% 				\dom\sDRS
% 			{}\ni{}
% 				u^k
% 			\),
% 			we have
			Then,
			\[
				\lambda[v^k-u^k]
			{}={}
				s^{k+1}-s^k
			{}={}
				\left[
					u^{k+1}-u^k
				\right]
				{}+{}
				\gamma
				\left[
					\Nabla\sDRS(u^{k+1})
					{}-{}
					\Nabla\sDRS(u^k)
				\right]
				{}+{}
				\nu^{k+1}-\nu^k.
			\]
			All the terms in square brackets belong to \(\dom\sDRS^\parallel\) whereas \(\nu^{k+1}-\nu^k\in\dom\sDRS^\perp\), and from the equation above we conclude that \(\nu^{k+1}-\nu^k=0\).
			Namely, there exists \(\nu\in\dom\sDRS^\perp\) (independent of the iteration \(k\in\N\)) such that
			\begin{equation}\label{eq:sznu}
				s^k
			{}={}
				u^k
				{}+{}
				\gamma\Nabla\sDRS(u^k)
				{}+{}
				\nu
			\qquad
				\text{for all \(k\in\N\).}
			\end{equation}
% 			However, since \(s^0\in\dom\sDRS\) we conclude that \(\nu=0\).
			Suppose now that \(\seq{u^k}[k\in K]\to u'\) for some \(K\subseteq\N\) and \(u'\in\R^p\).
			Then, \(\seq{v^k}[k\in K]\to u'\) and
			\(
				\seq{s^k}[k\in K]
			{}\to{}
				s'
			{}={}
				u'+\gamma\Nabla\sDRS(u')+\nu
			\),
			due to continuity of \(\Nabla\sDRS\) on \(\dom\sDRS\).
			From \cref{prop:proxfEquiv} we infer that \(u'=\prox_{\gamma\sDRS}(s')\).
			Therefore,
			\[
				v^k
			{}\in{}
				\prox_{\gamma\nsDRS}(2u^k-s^k)
			{}={}
				\prox_{\gamma\nsDRS}(\Fw{u^k}-\nu)
			{}={}
				\prox_{\gamma\nsDRS}(\Fw{u^k})
			\]
			where the last equality follows from \cref{prop:proxg}.
			Since \(\seq{\Fw{u^k}}[k\in K]\to \Fw{u'}\), the outer semicontinuity of \(\prox_{\gamma\nsDRS}\) \cite[Ex. 5.23(b)]{rockafellar2011variational} implies that
			\[
				u'
			{}={}
				\hspace*{-5pt}
				\lim_{K\ni k\to\infty}{
					\hspace*{-5pt}
					u^k
				}
			{}\in{}
				\limsup_{K\ni k\to\infty}{
					\FB{u^k}
				}
			{}\subseteq{}
				\FB{u'}.
			\]
			From the optimality of \(u'\in\FB{u'}\) it follows that \(u'\) minimizes
			\(
				\psi
			{}\coloneqq{}
				\nsDRS
				{}+{}
				\tfrac{1}{2\gamma}
				\|
					{}\cdot{}
					{}-{}
					u'+\gamma\Nabla\sDRS(u')
				\|^2
			\),
			and therefore
			\[
				0
			{}\in{}
				\hat\partial\psi(u')
			{}={}
				\hat\partial\nsDRS(u')
				{}+{}
				\tfrac1\gamma(u'-u'+\gamma\Nabla\sDRS(u'))
			{}\subseteq{}
				\hat\partial\varphi(u')
			\]
			where the first equality follows from \cite[Thm. 10.1]{rockafellar2011variational} and the last inclusion from \eqref{eq:partialf}.
			Finally, since \(v^k\to v'\),
			\[
				\varphi(u')
			{}\leq{}
				\liminf_{K\ni k\to\infty}{
					\varphi(v^k)
				}
			{}\leq{}
				\limsup_{K\ni k\to\infty}{
					\varphi(v^k)
				}
			{}\leq{}
				\limsup_{K\ni k\to\infty}{
					\DRE(s^k)
				}
			{}={}
				\DRE(s')
			{}\leq{}
				\varphi(u')
			\]
			where in the first inequality we used lower semicontinuity of \(\varphi\), in the third and last the sandwiching property (\cref{prop:sandwich}), and in the equality the continuity of \(\DRE\).
			This shows that \(\seq{\varphi(u^k)}[k\in K]\to\varphi(u')=\DRE(s')\), and since \(\seq{\DRE(s^k)}\to\varphi_\star\), then necessarily \(\varphi(u')=\DRE(s')=\varphi_\star\) independently of the cluster point \(u'\).
		\end{proofitemize}
		Finally, suppose that \(\varphi\) has bouneded level sets.
		Then, it follows from \cref{prop:boundedlev} that so does \(\DRE\), and since \(s^k\in\lev_{\leq\DRE(s^0)}\DRE\) for all \(k\in\N\), then the sequence \(\seq{s^k}\) is bounded.
		From Lipschitz continuity of \(\prox_{\gamma\sDRS}\) (cf. \cref{prop:proxfLip}) it then follow that also \(\seq{u^k}\) is bounded and since \(v^k-u^k\to 0\) we conclude that so is \(\seq{v^k}\).
	\end{proof}
\end{thm}

\begin{grayout}
	\begin{thm}[Global convergence of \ref{DRS}]\label{thm:DRSglobal}%
		Suppose that \(\varphi\) has bounded level sets, and consider the iterates generated by \ref{DRS}.
		Let \(\omega\) denote the set of cluster points of the sequence \(\seq{s^k}\), and suppose that for all \(\bar x=\prox_{\gamma\sDRS}(\bar s)\) with \(\bar s\in\omega\) the following hold:
		\begin{enumass}
		\item
			\(\restr{\sDRS}\) is \(\cont^2\) in a neighborhood of \(\bar x\);
		\item
			\(\nsDRS\) is prox-regular at \(\bar x\) for \(-\Nabla\sDRS(\bar x)\);
		\item
			\(\DRE\) possesses the KL-property at \(\bar s\).
		\end{enumass}
		Then, there exists \(s^\star\) such that \(s^k\to s^\star\) (in particular, \(\omega=\set{s^\star}\)).
		\begin{proof}
			To avoid trivialities, we assume that \(v^k\neq u^k\) for all \(k\in\N\).
			We know from \cref{thm:DRS} that \(\seq{s^k}\) remains bounded and therefore \(\omega\neq\emptyset\).
			Moreover, \cref{prop:C1} ensures that \(\DRE\) is continuously differentiable in a neighborhood of \(\omega\) with
			\[
				\nabla\DRE(s)
			{}={}
				\tfrac1\gamma
				J\prox_{\gamma\sDRS}(s)
				Q_\gamma(u)(u-v)
			\]
			where
			\(
				Q_\gamma
			{}\coloneqq{}
				\I-\gamma\Nabla^2\sDRS
			\).
			It follows from \cref{prop:proxfLip} that for all \(x\in\dom\sDRS\)
			\(
				\tfrac{1}{1+\gamma L_{\sDRS}}
				\|x\|^2
			{}\leq{}
				\innprod{x}{J\prox_{\gamma\sDRS}(s)x}
			{}\leq{}
				\tfrac{1}{1+\gamma\sigma_{\sDRS}}
				\|x\|^2
			\);
			since \(Q_\gamma(u)(u-v)\in\dom\sDRS\) and
			\(
				(1+\gamma\sigma_{\sDRS})\I
			{}\preceq{}
				Q_\gamma(u)
			{}\preceq{}
				(1+\gamma L_{\sDRS})\I
			\),
			we conclude that
			\begin{equation}\label{eq:nablaBounds}
				\tfrac{1+\gamma\sigma_{\sDRS}}{\sqrt{1+\gamma L_{\sDRS}}}
				\|u^k-v^k\|
			{}\leq{}
				\|\nabla\DRE(s^k)\|
			{}\leq{}
				\tfrac{1+\gamma L_{\sDRS}}{\sqrt{1+\gamma\sigma_{\sDRS}}}
				\|u^k-v^k\|.
			\end{equation}
			Moreover, it follows from \cref{thm:DRN} that \(\DRE(s^k)\searrow\varphi_\star\equiv\restr{\DRE}[\omega]\) for some \(\varphi_\star\in\R\), and since \(s^{k+1}-s^k=\lambda(v^k-u^k)\to0\), \cite[Rem. 5]{bolte2014proximal} ensures that \(\omega\) is a nonempty compact and connected set such that \(\dist(s^k,\omega)\to 0\).
			Then, from \cite[Lem. 6]{bolte2014proximal} we conclude that \(\DRE\) enjoys the \emph{uniform KL-property} on \(\omega\).
			Namely, there exist \(\varepsilon,\eta>0\), an open set \(\mathcal U\supset\omega\) and a continuous concave function \(\func{\psi}{[0,\eta)}{[0,+\infty)}\) such that \(\psi(0)=0\), \(\psi\) is \(\cont^1\) with \(\psi'>0\) on \((0,\eta)\), and
			\[
				\psi'(\DRE(s)-\varphi_\star)
				\|\nabla\DRE(s)\|
			{}\geq{}
				1
			\quad
				\text{for all \(s\in\mathcal U\) such that }
				\varphi_\star
			{}<{}
				\DRE(s)
			{}<{}
				\varphi_\star+\varepsilon
			\]
			(\(\mathcal U\) is taken small enough such that \(\DRE\) is \(\cont^1\) on \(\mathcal U\), hence the notation \(\nabla\DRE\) is legit).
			Since \(\dist(s^k,\omega)\to 0\), \(\DRE(s^k)\searrow\varphi_\star\) and \(\DRE(s^k)\neq\varphi_\star\) (due to the sufficient decrease, cf. \eqref{eq:SD}), there exists some \(\bar k\in\N\) such that
			\(
				\dist(s^k,\omega)
			{}<{}
				\varepsilon
			\)
			and
			\(
				\varphi_\star
			{}<{}
				\DRE(s^k)
			{}<{}
				\varphi_\star+\varepsilon
			\)
			for all \(k\geq\bar k\).
			Let
			\(
				\Delta_k
			{}\coloneqq{}
				\psi(\DRE(s^k)-\varphi_\star)
			\);
			then, due to concavity of \(\psi\) we have
			\begin{align*}
				\Delta_k
				{}-{}
				\Delta_{k+1}
			{}\geq{} &
				\psi'(\DRE(s^k)-\varphi_\star)
				(\DRE(s^k)-\DRE(s^{k+1}))
			{}\geq{}
				c
				\frac{
					\|u^k-v^k\|\mathrlap{^2}
				}{
					\|\nabla\DRE(s^k)\|
				}
			\\
			{}\overrel[\geq]{\eqref{eq:nablaBounds}}{} &
				c
				\tfrac{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}{
					1+\gamma L_{\sDRS}
				}
				\|u^k-v^k\|
			{}={}
				\tfrac{c}{\lambda}
				\tfrac{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}{
					1+\gamma L_{\sDRS}
				}
				\|s^k-s^{k+1}\|
			\end{align*}
			where the last inequality follows from the identity
			\(
				s^{k+1}-s^k
			{}={}
				\lambda(v^k-u^k)
			\).
			Therefore,
			\[
				\sum_{k\geq\bar k}{
					\|s^k-s^{k+1}\|
				}
			{}\leq{}
				\tfrac{\lambda}{c}
				\tfrac{
					1+\gamma L_{\sDRS}
				}{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}
				\sum_{k\geq\bar k}{\left(
					\Delta_k
					{}-{}
					\Delta_{k+1}
				\right)}
			{}\leq{}
				\tfrac{\lambda}{c}
				\tfrac{
					1+\gamma L_{\sDRS}
				}{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}
				\Delta_{\bar k}
			{}<{}
				\infty,
			\]
			that is, \(\seq{s^k}\) has finite length and therefore is convergent.
		\end{proof}
	\end{thm}
\end{grayout}


==> TeX/Text/DRS/Convergence.tex <==
\begin{thm}[Subsequential convergence]\label{thm:DRS}%
	Suppose that the cost function \(\varphi\) is lower bounded.
	Then, the following hold for the iterates generated by \ref{DRS} with stepsize \(\gamma\) and relaxation \(\lambda\) as in \Cref{thm:SD}:
	\begin{enumerate}
	\item\label{thm:DRS:r}
		the sequence of DR-residuals \(\seq{u^k-v^k}\) is square-summable;
	\item\label{thm:DRS:uv}
		\(\seq{u^k}\) and \(\seq{v^k}\) have same cluster points, all of which are stationary for \(\varphi\) and on which \(\varphi\) has same value, this being the limit of \(\seq{\DRE(s^k)}\).
	\end{enumerate}
	Moreover, a sufficient condition for the sequences to be bounded is that \(\varphi\) has bounded level sets.
	\begin{proof}
		To avoid trivialities, we assume that the stopping criterion \(v^k=u^k\) is never met, so that the algorithm runs infinite many iterations.
		\begin{proofitemize}
		\item\ref{thm:DRS:r}
			Let \(c=c(\gamma,\lambda)\) be as in \cref{thm:SD}.
			Telescoping the inequality \eqref{eq:SD} yields
			\begin{align*}
			\textstyle
				c
				\sum_{k\in\N}{
					\|u^k-v^k\|^2
				}
			{}\leq{} &
			\textstyle
				\sum_{k\in\N}{
				\bigl[
					\DRE(s^k)
					{}-{}
					\DRE(s^{k+1})
				\bigr]}
			{}\leq{}
				\DRE(s^0)-\inf\DRE.
			\end{align*}
			Since \(\inf\DRE=\inf\varphi\) and \(\DRE\) is real-valued (cf. \cref{prop:C0,prop:DREequiv}), from the inequality above it follows that if \(\varphi\) is lower bounded then \(\seq{u^k-v^k}\) is square-summable.
			Moreover, since \(\DRE(s^k)\) is decreasing it admits a limit, be it \(\varphi_\star>-\infty\).
	%%%%%%%%
		\item\ref{thm:DRS:uv}
			Since \(\seq{u^k-v^k}\to 0\), necessarily \(\seq{u^k}\) and \(\seq{v^k}\) have same cluster points.
			From \cref{prop:proxfEquiv} it follows that for all \(k\in\N\)
			there exists \(\nu^k\in\dom\sDRS^\perp\) such that
			\(
				s^k
			{}={}
				u^k+\gamma\Nabla\sDRS(u^k)+\nu^k
			\).
% 			However, since
% 			\(
% 				v^k
% 			{}\in{}
% 				\dom\nsDRS
% 			{}\subseteq{}
% 				\dom\sDRS
% 			{}\ni{}
% 				u^k
% 			\),
% 			we have
			Then,
			\[
				\lambda[v^k-u^k]
			{}={}
				s^{k+1}-s^k
			{}={}
				\left[
					u^{k+1}-u^k
				\right]
				{}+{}
				\gamma
				\left[
					\Nabla\sDRS(u^{k+1})
					{}-{}
					\Nabla\sDRS(u^k)
				\right]
				{}+{}
				\nu^{k+1}-\nu^k.
			\]
			All the terms in square brackets belong to \(\dom\sDRS^\parallel\) whereas \(\nu^{k+1}-\nu^k\in\dom\sDRS^\perp\), and from the equation above we conclude that \(\nu^{k+1}-\nu^k=0\).
			Namely, there exists \(\nu\in\dom\sDRS^\perp\) (independent of the iteration \(k\in\N\)) such that
			\begin{equation}\label{eq:sznu}
				s^k
			{}={}
				u^k
				{}+{}
				\gamma\Nabla\sDRS(u^k)
				{}+{}
				\nu
			\qquad
				\text{for all \(k\in\N\).}
			\end{equation}
% 			However, since \(s^0\in\dom\sDRS\) we conclude that \(\nu=0\).
			Suppose now that \(\seq{u^k}[k\in K]\to u'\) for some \(K\subseteq\N\) and \(u'\in\R^p\).
			Then, \(\seq{v^k}[k\in K]\to u'\) and
			\(
				\seq{s^k}[k\in K]
			{}\to{}
				s'
			{}={}
				u'+\gamma\Nabla\sDRS(u')+\nu
			\),
			due to continuity of \(\Nabla\sDRS\) on \(\dom\sDRS\).
			From \cref{prop:proxfEquiv} we infer that \(u'=\prox_{\gamma\sDRS}(s')\).
			Therefore,
			\[
				v^k
			{}\in{}
				\prox_{\gamma\nsDRS}(2u^k-s^k)
			{}={}
				\prox_{\gamma\nsDRS}(\Fw{u^k}-\nu)
			{}={}
				\prox_{\gamma\nsDRS}(\Fw{u^k})
			\]
			where the last equality follows from \cref{prop:proxg}.
			Since \(\seq{\Fw{u^k}}[k\in K]\to \Fw{u'}\), the outer semicontinuity of \(\prox_{\gamma\nsDRS}\) \cite[Ex. 5.23(b)]{rockafellar2011variational} implies that
			\[
				u'
			{}={}
				\hspace*{-5pt}
				\lim_{K\ni k\to\infty}{
					\hspace*{-5pt}
					u^k
				}
			{}\in{}
				\limsup_{K\ni k\to\infty}{
					\FB{u^k}
				}
			{}\subseteq{}
				\FB{u'}.
			\]
			From the optimality of \(u'\in\FB{u'}\) it follows that \(u'\) minimizes
			\(
				\psi
			{}\coloneqq{}
				\nsDRS
				{}+{}
				\tfrac{1}{2\gamma}
				\|
					{}\cdot{}
					{}-{}
					u'+\gamma\Nabla\sDRS(u')
				\|^2
			\),
			and therefore
			\[
				0
			{}\in{}
				\hat\partial\psi(u')
			{}={}
				\hat\partial\nsDRS(u')
				{}+{}
				\tfrac1\gamma(u'-u'+\gamma\Nabla\sDRS(u'))
			{}\subseteq{}
				\hat\partial\varphi(u')
			\]
			where the first equality follows from \cite[Thm. 10.1]{rockafellar2011variational} and the last inclusion from \eqref{eq:partialf}.
			Finally, since \(v^k\to v'\),
			\[
				\varphi(u')
			{}\leq{}
				\liminf_{K\ni k\to\infty}{
					\varphi(v^k)
				}
			{}\leq{}
				\limsup_{K\ni k\to\infty}{
					\varphi(v^k)
				}
			{}\leq{}
				\limsup_{K\ni k\to\infty}{
					\DRE(s^k)
				}
			{}={}
				\DRE(s')
			{}\leq{}
				\varphi(u')
			\]
			where in the first inequality we used lower semicontinuity of \(\varphi\), in the third and last the sandwiching property (\cref{prop:sandwich}), and in the equality the continuity of \(\DRE\).
			This shows that \(\seq{\varphi(u^k)}[k\in K]\to\varphi(u')=\DRE(s')\), and since \(\seq{\DRE(s^k)}\to\varphi_\star\), then necessarily \(\varphi(u')=\DRE(s')=\varphi_\star\) independently of the cluster point \(u'\).
		\end{proofitemize}
		Finally, suppose that \(\varphi\) has bouneded level sets.
		Then, it follows from \cref{prop:boundedlev} that so does \(\DRE\), and since \(s^k\in\lev_{\leq\DRE(s^0)}\DRE\) for all \(k\in\N\), then the sequence \(\seq{s^k}\) is bounded.
		From Lipschitz continuity of \(\prox_{\gamma\sDRS}\) (cf. \cref{prop:proxfLip}) it then follow that also \(\seq{u^k}\) is bounded and since \(v^k-u^k\to 0\) we conclude that so is \(\seq{v^k}\).
	\end{proof}
\end{thm}

\begin{grayout}
	\begin{thm}[Global convergence of \ref{DRS}]\label{thm:DRSglobal}%
		Suppose that \(\varphi\) has bounded level sets, and consider the iterates generated by \ref{DRS}.
		Let \(\omega\) denote the set of cluster points of the sequence \(\seq{s^k}\), and suppose that for all \(\bar x=\prox_{\gamma\sDRS}(\bar s)\) with \(\bar s\in\omega\) the following hold:
		\begin{enumass}
		\item
			\(\restr{\sDRS}\) is \(\cont^2\) in a neighborhood of \(\bar x\);
		\item
			\(\nsDRS\) is prox-regular at \(\bar x\) for \(-\Nabla\sDRS(\bar x)\);
		\item
			\(\DRE\) possesses the KL-property at \(\bar s\).
		\end{enumass}
		Then, there exists \(s^\star\) such that \(s^k\to s^\star\) (in particular, \(\omega=\set{s^\star}\)).
		\begin{proof}
			To avoid trivialities, we assume that \(v^k\neq u^k\) for all \(k\in\N\).
			We know from \cref{thm:DRS} that \(\seq{s^k}\) remains bounded and therefore \(\omega\neq\emptyset\).
			Moreover, \cref{prop:C1} ensures that \(\DRE\) is continuously differentiable in a neighborhood of \(\omega\) with
			\[
				\nabla\DRE(s)
			{}={}
				\tfrac1\gamma
				J\prox_{\gamma\sDRS}(s)
				Q_\gamma(u)(u-v)
			\]
			where
			\(
				Q_\gamma
			{}\coloneqq{}
				\I-\gamma\Nabla^2\sDRS
			\).
			It follows from \cref{prop:proxfLip} that for all \(x\in\dom\sDRS\)
			\(
				\tfrac{1}{1+\gamma L_{\sDRS}}
				\|x\|^2
			{}\leq{}
				\innprod{x}{J\prox_{\gamma\sDRS}(s)x}
			{}\leq{}
				\tfrac{1}{1+\gamma\sigma_{\sDRS}}
				\|x\|^2
			\);
			since \(Q_\gamma(u)(u-v)\in\dom\sDRS\) and
			\(
				(1+\gamma\sigma_{\sDRS})\I
			{}\preceq{}
				Q_\gamma(u)
			{}\preceq{}
				(1+\gamma L_{\sDRS})\I
			\),
			we conclude that
			\begin{equation}\label{eq:nablaBounds}
				\tfrac{1+\gamma\sigma_{\sDRS}}{\sqrt{1+\gamma L_{\sDRS}}}
				\|u^k-v^k\|
			{}\leq{}
				\|\nabla\DRE(s^k)\|
			{}\leq{}
				\tfrac{1+\gamma L_{\sDRS}}{\sqrt{1+\gamma\sigma_{\sDRS}}}
				\|u^k-v^k\|.
			\end{equation}
			Moreover, it follows from \cref{thm:DRN} that \(\DRE(s^k)\searrow\varphi_\star\equiv\restr{\DRE}[\omega]\) for some \(\varphi_\star\in\R\), and since \(s^{k+1}-s^k=\lambda(v^k-u^k)\to0\), \cite[Rem. 5]{bolte2014proximal} ensures that \(\omega\) is a nonempty compact and connected set such that \(\dist(s^k,\omega)\to 0\).
			Then, from \cite[Lem. 6]{bolte2014proximal} we conclude that \(\DRE\) enjoys the \emph{uniform KL-property} on \(\omega\).
			Namely, there exist \(\varepsilon,\eta>0\), an open set \(\mathcal U\supset\omega\) and a continuous concave function \(\func{\psi}{[0,\eta)}{[0,+\infty)}\) such that \(\psi(0)=0\), \(\psi\) is \(\cont^1\) with \(\psi'>0\) on \((0,\eta)\), and
			\[
				\psi'(\DRE(s)-\varphi_\star)
				\|\nabla\DRE(s)\|
			{}\geq{}
				1
			\quad
				\text{for all \(s\in\mathcal U\) such that }
				\varphi_\star
			{}<{}
				\DRE(s)
			{}<{}
				\varphi_\star+\varepsilon
			\]
			(\(\mathcal U\) is taken small enough such that \(\DRE\) is \(\cont^1\) on \(\mathcal U\), hence the notation \(\nabla\DRE\) is legit).
			Since \(\dist(s^k,\omega)\to 0\), \(\DRE(s^k)\searrow\varphi_\star\) and \(\DRE(s^k)\neq\varphi_\star\) (due to the sufficient decrease, cf. \eqref{eq:SD}), there exists some \(\bar k\in\N\) such that
			\(
				\dist(s^k,\omega)
			{}<{}
				\varepsilon
			\)
			and
			\(
				\varphi_\star
			{}<{}
				\DRE(s^k)
			{}<{}
				\varphi_\star+\varepsilon
			\)
			for all \(k\geq\bar k\).
			Let
			\(
				\Delta_k
			{}\coloneqq{}
				\psi(\DRE(s^k)-\varphi_\star)
			\);
			then, due to concavity of \(\psi\) we have
			\begin{align*}
				\Delta_k
				{}-{}
				\Delta_{k+1}
			{}\geq{} &
				\psi'(\DRE(s^k)-\varphi_\star)
				(\DRE(s^k)-\DRE(s^{k+1}))
			{}\geq{}
				c
				\frac{
					\|u^k-v^k\|\mathrlap{^2}
				}{
					\|\nabla\DRE(s^k)\|
				}
			\\
			{}\overrel[\geq]{\eqref{eq:nablaBounds}}{} &
				c
				\tfrac{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}{
					1+\gamma L_{\sDRS}
				}
				\|u^k-v^k\|
			{}={}
				\tfrac{c}{\lambda}
				\tfrac{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}{
					1+\gamma L_{\sDRS}
				}
				\|s^k-s^{k+1}\|
			\end{align*}
			where the last inequality follows from the identity
			\(
				s^{k+1}-s^k
			{}={}
				\lambda(v^k-u^k)
			\).
			Therefore,
			\[
				\sum_{k\geq\bar k}{
					\|s^k-s^{k+1}\|
				}
			{}\leq{}
				\tfrac{\lambda}{c}
				\tfrac{
					1+\gamma L_{\sDRS}
				}{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}
				\sum_{k\geq\bar k}{\left(
					\Delta_k
					{}-{}
					\Delta_{k+1}
				\right)}
			{}\leq{}
				\tfrac{\lambda}{c}
				\tfrac{
					1+\gamma L_{\sDRS}
				}{
					\sqrt{1+\gamma\sigma_{\sDRS}}
				}
				\Delta_{\bar k}
			{}<{}
				\infty,
			\]
			that is, \(\seq{s^k}\) has finite length and therefore is convergent.
		\end{proof}
	\end{thm}
\end{grayout}

